AIM: An Adaptive and Iterative Mechanism for Differentially Private Synthetic Data

We propose AIM, a new algorithm for differentially private synthetic data generation. AIM is a workload-adaptive algorithm within the paradigm of algorithms that first selects a set of queries, then privately measures those queries, and finally generates synthetic data from the noisy measurements. It uses a set of innovative features to iteratively select the most useful measurements, reflecting both their relevance to the workload and their value in approximating the input data. We also provide analytic expressions to bound per-query error with high probability which can be used to construct confidence intervals and inform users about the accuracy of generated data. We show empirically that AIM consistently outperforms a wide variety of existing mechanisms across a variety of experimental settings.

==> discussion.tex <==
\revision{
\section{Discussion}

In this paper, we studied the problem of differentially private synthetic data generation, surveying the field and identifying strengths and weaknesses of prior work.  While much of the prior work is conceptually similar, details and specific design decisions differ from mechanism to mechanism, and these small differences can lead to large performance differences in practice.  In practical deployments of differential privacy, these details matter to obtain the best privacy-utility trade-off.  In this work, we propose \aim, a new mechanism where every detail is carefully thought out to work well in practice.  These details allowed \aim to consistently and significantly outperform competitors in our empirical evalaution.
}

==> fig1.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{fig/legend}
\subcaptionbox{\vspace{1em}Adult}{\includegraphics[width=0.335\textwidth]{fig/l1-adult-all3way}}
\subcaptionbox{Salary}{\includegraphics[width=0.318\textwidth]{fig/l1-salary-all3way}}
\subcaptionbox{MSNBC}{\includegraphics[width=0.318\textwidth]{fig/l1-msnbc-all3way}}
\subcaptionbox{Fire}{\includegraphics[width=0.335\textwidth]{fig/l1-fire-all3way}}
\subcaptionbox{NLTCS}{\includegraphics[width=0.318\textwidth]{fig/l1-nltcs-all3way}}
\subcaptionbox{Titanic}{\includegraphics[width=0.312\textwidth]{fig/l1-titanic-all3way}}
\caption{\label{fig:3way} Workload error of competing mechanisms on the \general workload for $\epsilon = 0.01, \dots, 100$.}
\end{figure*}


==> fig2.tex <==
\begin{figure*}[t!]
\centering
%\includegraphics[width=\textwidth]{fig/legend}
\subcaptionbox{Adult}{\includegraphics[width=0.335\textwidth]{fig/l1-adult-target}}
\subcaptionbox{Salary}{\includegraphics[width=0.318\textwidth]{fig/l1-salary-target}}
\subcaptionbox{MSNBC}{\includegraphics[width=0.318\textwidth]{fig/l1-msnbc-target}}
\subcaptionbox{Fire}{\includegraphics[width=0.335\textwidth]{fig/l1-fire-target}}
\subcaptionbox{NLTCS}{\includegraphics[width=0.318\textwidth]{fig/l1-nltcs-target}}
\subcaptionbox{Titanic}{\includegraphics[width=0.312\textwidth]{fig/l1-titanic-target}}
\caption{\label{fig:target} Workload error of competing mechanisms on the \target workload for $\epsilon = 0.01, \dots, 100$.}
\end{figure*}

==> fig3.tex <==
\begin{figure*}[t!]
\centering
%\includegraphics[width=\textwidth]{fig/legend}
\subcaptionbox{Adult}{\includegraphics[width=0.335\textwidth]{fig/l1-adult-weighted}}
\subcaptionbox{Salary}{\includegraphics[width=0.318\textwidth]{fig/l1-salary-weighted}}
\subcaptionbox{MSNBC}{\includegraphics[width=0.318\textwidth]{fig/l1-msnbc-weighted}}
\subcaptionbox{Fire}{\includegraphics[width=0.335\textwidth]{fig/l1-fire-weighted}}
\subcaptionbox{NLTCS}{\includegraphics[width=0.318\textwidth]{fig/l1-nltcs-weighted}}
\subcaptionbox{Titanic}{\includegraphics[width=0.312\textwidth]{fig/l1-titanic-weighted}}
\caption{\label{fig:weighted} Workload error of competing mechanisms on the \weighted workload for $\epsilon = 0.01, \dots, 100$.}
\end{figure*}


==> more_related.tex <==
\section{Related Work} \label{sec:more_related}

In \cref{sec:prior} we focused our discussion on \emph{marginal-based} mechanisms in the select-measure-generate paradigm.  While this is a popular approach, it is not the only way to generate differentially private synthetic data.  In this section we provide a brief discussion of other methods, and a broad overview of other relevant work.

One prominent approach is based on differentially private GANs.  Several architectures and private learning procedures have been proposed under this paradigm \cite{jordon2018pate,zhang2018differentially,tantipongpipat2019differentially,frigerio2019differentially,xie2018differentially,beaulieu2019privacy,abay2018privacy,torfi2020differentially,torkzadehmahani2019dp}.   Despite their popularity, we are not aware of evidence that these GAN-based mechanisms outperform even baseline marginal-based mechanisms like \privbayes on structured tabular data.  Most empirical evaluations of GAN-based mechanisms exclude \privbayes, and the comparisons that we are aware of show the opposite effect: that marginal-based mechanisms outperform the competition \cite{cai2021data, tao2021benchmarking, mckenna2021winning}.  GAN-based methods may be better suited for different data modalities such as image or text data.

One exception is CT-GAN \cite{xu2019modeling} which is an algorithm for synthetic data that compares well against \privbayes and outperforms it in roughly 85\% of the datasets and metrics they considered.  However, this method does not satisfy or claim to satisfy differential privacy and gives no formal privacy guarantee to the individuals who contribute data.
%Lacking formal privacy guarantees, the task of synthetic data lacks a clear and compelling motivation.
Nevertheless, an empirical comparison between CT-GAN and newer methods for synthetic data, like \aim and \privmrf, would be interesting, since these mechanisms also outperformed \privbayespgm in nearly every tested situation, and \privbayespgm outperforms \privbayes most of the time as well \cite{mckenna2019graphical,cai2021data}.  Differentially private implementations of CT-GAN have been proposed, but empirical evaluations of the method suggest it is not competitive with \privbayes \cite{rosenblatt2020differentially,tao2021benchmarking}.

%The high-dimensional matrix mechanism \cite{mckenna2018optimizing} (HDMM) is an algorithm for the related task of answering a workload of linear queries under differential privacy.  While this algorithm does provide answers to the workload queries, it generally does not produce synthetic data, unless combined with techniques like \pgm.  Even then, there are challenges to running it on very high-dimensional datasets, like the ones considered in this work.  The largest domain HDMM is capable of running on is roughly $10^9$, which is substantially smaller than the domains of the datasets we used in our empirical evaluation.  Moreover, while HDMM is a state-of-the-art data-independent mechanisms for workload query answering, simple data-dependent mechanisms can and do outperform it in many settings.  As $\epsilon$ tends to infinity, HDMM would be difficult to beat, but for modest values of epsilon data-dependent mechanisms are often better \cite{hay2016principled}.


==> related_old.tex <==
\section{Related Work}

\begin{algorithm}[tb]
    \caption{MWEM+PGM}
\begin{algorithmic}
    \STATE {\bfseries Input:} Dataset $D$, workload $W$, privacy parameter $\rho$, rounds $T$
    \STATE {\bfseries Output:} Synthetic Dataset $\hat{D}$
    \STATE Initialize $\hat{p}_0 = \text{Uniform}[\mathcal{X}] $
    \STATE $\epsilon = \sqrt{2 \rho / T}$
    \STATE $\sigma = \sqrt{T / \rho}$
    \FOR{$t = 1, \dots, T$}
        \STATE \textbf{select} $C \in W$ using quality score function:
$$ q(C; D) = || M_C(D) - M_C(\hat{p}_{t-1}) ||_1 - n_C $$
        \STATE \textbf{measure} marginal on $C$:
$$\tilde{y}_t = M_C(D) + \mathcal{N}(0, \sigma^2)^{n_{C}}$$
        \STATE \textbf{estimate} data distribution using \pgm:
$$ \hat{p_t} = \argmin_{p \in S} \sum_{y, \sigma, C} \frac{1}{\sigma} || M_C(p) - y ||_2^2 $$
    \ENDFOR
    \STATE \textbf{generate} synthetic data $\hat{D}$ using \pgm:
    \STATE {\bfseries return} $\hat{D}$
\end{algorithmic}
\end{algorithm}




\begin{algorithm}[tb]
    \caption{AIM: An Adaptive and Iterative Mechanism}
\begin{algorithmic}
    \STATE {\bfseries Input:} Dataset $D$, workload $W$, privacy parameter $\rho$
    \STATE {\bfseries Output:} Synthetic Dataset $\hat{D}$
    \STATE Initialize $\hat{p}_0 = \text{Uniform}[\mathcal{X}] $
    \STATE $T = 16 d$
    \STATE $\epsilon = \sqrt{8 \cdot 0.1 / 2 T}$
    \STATE $\sigma = \sqrt{T / (2 \cdot 0.8)}$
    \STATE $\rho_{used} = 0$
    \STATE $t = 0$
    \STATE $w(C) = \sum_{B \in W} \mid C \cap B \mid$
    \WHILE{$\rho_{used} < \rho$}
        \IF{$(\rho - \rho_{used}) \leq 2 \big( \frac{1}{2\sigma^2} + \frac{1}{8} \epsilon^2 \big)$}
            \STATE $\epsilon = \sqrt{8 \cdot 0.1 \cdot (\rho - \rho_{used})}$
            \STATE $\sigma = \sqrt{1 / (2 \cdot 0.9 \cdot (\rho - \rho_{used}))}$
        \ENDIF
        \STATE $\rho_{used} \leftarrow \rho_{used} + \frac{1}{8} \epsilon^2 + \frac{1}{2\sigma^2}$
        \STATE $t = t+1$
        \STATE candidates = $  \set{ C \in W_+ \mid \textsf{JT-SIZE}(C \cup \mathcal{C}) \leq \frac{\rho_{used}}{\rho} \cdot 100 \textsf{MB} }$
        \STATE \textbf{select} $C \in$ candidates using quality score function:
$$ q(C; D) = w(C) \Big( || M_C(D) - M_C(\hat{p}_{t-1}) ||_1 - \sqrt{2/\pi} \cdot \sigma \cdot n_C \Big) $$
        \STATE \textbf{measure} marginal on $C$:
$$\tilde{y}_t = M_C(D) + \mathcal{N}(0, \sigma^2)^{n_{C}}$$
        \STATE \textbf{estimate} data distribution using \pgm:
$$ \hat{p_t} = \argmin_{p \in S} \sum_{y, \sigma, C} \frac{1}{\sigma} || M_C(p) - y ||_2^2 $$
        \IF{$\norm{M_C(\hat{p}_t) - M_C(\hat{p}_{t-1})} \leq \sqrt{2/\pi} \cdot \sigma \cdot n_C$}
            \STATE $\epsilon \leftarrow 2 \cdot \epsilon $
            \STATE $\sigma \leftarrow \sigma / 2$
        \ENDIF
    \ENDWHILE
    \STATE \textbf{generate} synthetic data $\hat{D}$ using \pgm:
    \STATE {\bfseries return} $\hat{D}$
\end{algorithmic}
\end{algorithm}


In this section we survey the state of the field, describing similarities and differences between different mechanisms for the task of differentially private synthetic data.   We focus our attention on \emph{marginal-based approaches} to differentially private synthetic data in this section, and briefly discuss other approaches at the end.  

\paragraph*{\textbf{Traditional Methods for Batch Query Answering}}

There is a long history of work on differentially private batch query answering, which is closely related to the task we consider here.  There, the goal is to simply answer a workload of queries with low (ideally minimal) error subject to the constraint of differential privacy.  Here, our goal is to generate synthetic data such that is accurate with respect to the workload queries.  While closely related, these two tasks are different, and in general the latter problem can be much harder for certain workloads.  Indeed, it has been shown that 
under standard cryptographic assumptions, generating differentially private synthetic data that preserves all 2-way marginals is computationally hard in the worst case, even though we can easily answer these queries with a simple invocation of the Gaussian mechanism \cite{ullman?}.  


\paragraph*{\textbf{HDMM}}

The High-Dimensional Matrix Mechanism (HDMM) is a mechanism for answering a workload of linear counting queries under differential privacy.  It is specifically designed to handle multi-dimensional domains and supports the expressive class of conjunctive query workloads we consider here.  HDMM is state-of-the-art algorithm for linear query answering in the large data, large $\epsilon$ regime.  However, there are a few limitations of HDMM that prevent it from being a viable method for synthetic data generation on high-dimensional domains.

First, HDMM requires materializing a data vector whose size is equal to the size of the domain, and is intractable to write down for high-dimensional domains.  This prevents us from running HDMM at all for many datasets with intractably large data vectors. \footnote{The name ``high-dimensional`` matrix mechanism is a a bit of a misnomer, since it fails to scale to high-dimensional domains.  It can scale up to extremely high-dimensional data vectors (up to size $10^9$), but many high-dimensional datasets have domains far larger than this.}  

Second, HDMM is a mechanism for linear query asnwering, not synthetic data generation.  It will produce estimated answers to the queries, but not provide synthetic data that produces those query answers.  While it does return a vector that contains estimated counts for each element of the data domain (and can be used to ansewr the queries), this vector could contain negative and non-integral values, whereas the true data vector would need to contain only negative and integral counts.  

Third, HDMM produces unbiased answers to the workload queries.  For large workloads, this property of HDMM requires it to measure an inordinate number of marginals, leading to an excessive amount of noise.  In the large data, large $\epsilon$ regime, this might be acceptable and even desired (such as the U.S. Census use case), but in the small data, low $\epsilon$ regime, HDMM can be outperformed by trivial baseline algorithms.  In such cases, it's often better to accept some bias in the workload query answers in order to reduce variance and overall error.  

HDMM can be integrated with \pgm to overcome the first two problems, while also improving it's performance in the small data, low $\epsilon$ regime.  Indeeed, this has been shown to allow HDMM to run in higher-dimensional domains than it was intended, while simultaneously improving it's error \cite{?,?}.  However, there are certain workloads, such as the workload of all 2-way marginals, where HDMM+\pgm simply fails to scale.  This violates our desiderata that run in a reasonable amount of time for any discrete dataset and workload satisfying our requirements.  

While HDMM is not a viable method by itself, we will utilize the technique as a subroutine in the mechanism we propose, allowing our method to enjoy the benefits HDMM in situations where it was intended to be used. 

\paragraph*{\textbf{Independent}}

The Independent mechanism is a very simple mechanism for synthetic data that is easy to implement and also provides a reasonable baseline for comparison of more sophisticated mechanisms.  To our knowledge, this mechanism has not been proposed in any published work we are aware of, although variants of this mechanism have been used with some success in the NIST synthetic data challenges.  In fact, these mechanisms won fourth place in both the 2018 challenge and 2020 challenge, even outperforming teams using GAN-based approaches.  The basic idea is to measure all 1-way marginals using a noise addition mechanism (Laplace/Gaussian).  We can then generate synthetic records for each column \emph{independently} from these noisy 1-way marginals, producing synthetic data.  

Despite it's simplicity, this mechanism is a strong baseline, especially in the small data, low $\epsilon$ regime.  Because it measures only $d$ marginals, it requires a modest amount of noise to preserve privacy.  However, since it only measures 1-way marginals, this mechanism does not preserve correlations between attributes or adapt the workload.  

\paragraph*{\textbf{MWEM}} 

Like HDMM, MWEM was originally proposed as a mechanism for batch query answering rather than synthetic data generation.  However, as a by-product of the algorithm, MWEM produces an estimate of the data distribution, which can be used to obtain synthetic data if desired.  However, MWEM represents this data distribution explicilty in vector form, which is intractable for high-dimensional data.  For this reason, MWEM by itself is not a viable method for synthetic data generation.  Unlike HDMM, MWEM does not try to produce unbiased answers to the workload queries.  Instead, it tries to identify a set of the most important queries, and answers those, accepting bias on the other queries.  By selecting a small subset of the workload queries to answer, MWEM saves privacy budget, allowing it to add less noise to the queries it does answer.  

A scalable implementation of MWEM was proposed in the original paper, demonstrating scaling capabilities up to $1000$-dimensional datasets.  However, this was achieved for a very special workload where queries could be partitioned into groups involving non-overlapping attributes.  For more complicated workloads with overlapping structure, the resource requirements required by this scalable implementation of MWEM approaches the ordinary version very quickly as the number of rounds of MWEM increases.  

\paragraph*{\textbf{MWEM+PGM}}

\paragraph*{\textbf{RAP}}

\paragraph*{\textbf{GEM}}

\paragraph*{\textbf{PrivBayes}}

\paragraph*{\textbf{JunctionTree}}

\paragraph*{\textbf{PrivSyn}}

\paragraph*{\textbf{PrivMRF}}

\paragraph*{\textbf{MST}}

\paragraph*{\textbf{Others}}

DualQuery, FEM, PMWPUB, Copula, GAN-based

\paragraph*{\textbf{Summary}}


==> response.tex <==

\section*{Reviewer Response}

We thank the reviewers for recognizing the strengths of the paper and offering insightful feedback and suggestions to improve it.  In the paragraphs below, we respond to the reviewer comments and summarize the changes made to the paper to address the concerns. All changes in the revised submission are \revision{highlighted in pink}.  In order to make space for the new additions, we removed discussion of GAN-based mechanisms in the additional related work section, and moved the experiments involing the model-capacity parameter to the \cref{sec:capacity}.  Some of the new experiments we conducted in revision also did not fit in the main body of the paper, but we added the important conclusions from these experiments and references to a full version where complete results and discussion can be found.  

\paragraph*{\textbf{[R1, R2] Ablation Study}}

We agree with the reviewers that an ablation study was an important missing piece from the version of the paper we originally submitted.  We added Section 6.5 to the paper, which carefully evaluates the impact of each element of AIM, including the basic elements of a good mechanism described in Section 3.2, as well as the new elements of AIM described in Section 4.  This analysis reveals that all of the elements together contribute to the strong performance of AIM, and measures the relative impact of each element.

\paragraph*{\textbf{[MR, R2] Default Parameter Settings}} 

In response to this concern, we conducted sensitivity experiments which now appear in \cref{sec:sensitivity} of our full paper, which evaluate the impact of hyper-parameters on the performance of competing mechanisms.  Our experimental results show that the improvement in utility from optimizing hyper-parameters is outweighed by the cost to privacy needed to run an appropriate DP hyper-parameter selection mechanism.  Therefore, it is actually better to use the default hyper-parameters than to perform hyper-parmaeter optimization in real-world deployments.  Additionally, even with a (non-private) hyper-parameter selection oracle, the gain in utility obtained from tuned hyper-parameters is not enough to meaningfully change any of our experimental findings.

\paragraph*{\textbf{[R1, R2] Notation Table}}

We added \cref{table:notation} to \cref{sec:background}, which lists notation used in the paper together with short descriptions.  

\paragraph*{\textbf{[R1, R2] Other workloads (non 3-way)}}

We conducted additional experiments on the workload of \workload{all-2way} marginals, and added them to \cref{sec:2way} of the full paper.  This new workload further confirms the experimental findings from the \general workload we considered in the main paper.

\paragraph*{\textbf{[R2] Limitations}}

We expanded our discussion of the limitations of \aim in \cref{sec:open}, by adding three new paragraphs, including one that discusses the granularity of our uncertainty quantification guarantees.  The reviewer is correct that our guarantees are with respect to the $L_1$ error of marginals in the workload, although finer grained guarantees relating to the error in each cell of the marginal could be useful in some applications.  

\paragraph*{\textbf{[R2] Other error metrics}}

The reviewer raises a good point about our use of the $L_1$ error metric in this work, and that $L_2$ and max error would also have been possible.  We now better motivate the use of the $L_1$ metric at the end of \cref{sec:workload}.  In addition, we added figures to \cref{sec:metrics} showing the performance of the mechanisms under these other metrics.  \aim is still the best-performing mechanism with respect to these metrics under many of the experimental settings considered, even though \aim is specifically designed to work well for $L_1$ error.  For max error, there are two datasets where \aim is outperformed by \gem, which is a mechanism specifically designed for max error.  A discussion of these results is included in \cref{sec:metrics}.

% \paragraph*{\textbf{[R2] Depth of contributions}}

% \ry{please fill in @Dan Sheldon, otherwise delete this paragraph}
% % : short positive paragraph, why it’s important.  Ignore negative points


\paragraph*{\textbf{[R2] Is initialization a contribution?}}

We added a sentence to \cref{sec:aim} to better justify this design decision.  We studied the impact of this element of \aim in \cref{sec:ablation}, and show that independent initialization has a modest, but statistically significant, positive effect on the performance of \aim, reducing error by a factor of $1.03$ on average (and up to $2.04$ in the best case) compared to the alternative uniform initialization.  The ``MWEM-style'' alternative (adding noise to each domain element) mentioned by the reviewer is infeasible for the datasets we considered, as the domains are too large to materialize the required histogram explicitly.  That idea is mainly applicable for lower-dimensional settings like 1- and 2-dimensional range query workloads, and marginal query workloads over smaller domains.  

\paragraph*{\textbf{[R2] Is the change in exponential mechanism quality function important?}}

As shown in our new ablation study in \cref{sec:ablation}, the new selection criteria + candidate set is indeed an important element of \aim, reducing error of the mechanism by $1.37\times$ on average compared to the alternative of using the selection criteria + candidate set from \mwempgm.

\paragraph*{\textbf{[R2] How important is budget annealing?}}

The reviewer's intuition is indeed correct that budget annealing is one of the more important elements of AIM, as shown in our new ablation study (\cref{sec:ablation}).  Compared to the alternative of running \aim for $d$ rounds (where $d$ is the number of attributes), \aim with adaptive rounds + budget split offers a $1.48\times$ improvement on average.  Moreover, \aim with this element is also better than \aim with a fixed number of rounds $T$ for $T = \set{2, 4, 8, 16, 32, 64, 128, 256, d}$, across all experimental settings (\cref{sec:adaptive}).  If, however, we optimally select $T$ for each individual experimental setting (dataset, workload, privacy budget) in a non-private manner, then this is indeed better than \aim with adaptive rounds + budget split.  On average, the error using the \emph{best T in hindsight} is only $1.1 \times$ better than \aim with adaptive rounds + budget split. Of course, using the best $T$ in hindsight would be a privacy violation, and so this would not be a feasible approach to use in real-world deployments.  

\paragraph*{\textbf{[R2] Novelty of Uncertainty Quantification Guarantees}}

In the introduction, we highlight both the potential and the peril of private synthetic data---it can be used to answer any query, but is necessarily limited in the number of queries it can answer accurately. As such, it is essential to develop tools that allow a user to know which queries can be answered accurately. We provide easy-to-compute post-hoc bounds on the error of different marginal queries.
% Users of private synthetic data can use these bounds directly to know whether the data can give accurate answers to give different queries.
We are not aware of any prior synthetic data mechanism that has provided similar bounds; we therefore consider them both novel and practically significant. In addition, there is technical novelty in their development, even though they use well known ingredients.  Nevertheless, we do not view the novelty of the analysis as the primary contribution.

\paragraph*{\textbf{[R2] Uses Cases for Uncertainty Quantification Guarantees}}

We added more discussion and references to better motivate the need for uncertainty quantification to \cref{sec:intro,sec:uncertainty}.  

\paragraph*{\textbf{[R2] Discussion of Uncertainty Quantification Guarantees}}

The reviewer correctly points out that in \cref{cor:supported1}, the bound on error of the synthetic data is worse than the bound on error for the noisy marginal, suggesting the synthetic data should be ignored in favor of the noisy measurements if the most accurate marginals are desired.  This is an interesting observation that warrants more discussion and clarification, which we now include after \cref{cor:supported1} in the revised paper.

\paragraph*{\textbf{[R2] Depth of experimental evaluation}}

We agree with the reviewer's observation that ``Every paper on synthetic data generation always shows that it outperforms the competitors'', and this is one reason that motivated us to pursue this research.  First, we saw clear sub-optimalities in existing work (see \cref{sec:basic,sec:distinguishing,sec:otherconsiderations}) that we felt needed to be addressed.  Second, several existing empirical evaluations were lacking, and failed to compare against state-of-the-art techniques (hence why they appeared to out-perform competitors).  One goal with our empirical evaluation was to compare mechanisms that had previously never been compared.  Indeed, our experimental evaluation revealed several interesting insights about existing work, e.g., the best workload-agnostic mechanism outperforms all existing workload-aware mechanisms across a variety of experimental settings -- a finding which until now was not known because the relevant experiments had not been conducted.

We differ with the reviewer's claim that we only ``show improved performance on a small set of data and workloads''.  Our experimental setup included $6$ datasets $\times$ $3$ workloads $\times$ $9$ privacy levels = $162$ experimental configurations, and AIM consistently outperformed $8$ other competitors in all of these settings.  This is significantly more comprehensive than experiments from prior work on this topic, some of which only include $2$ datasets, $2$ workloads, a narrow range of privacy levels (often only between $0.1$ and $1.0$), and limited competing mechanisms \cite{vietri2020new,aydore2021differentially,liu2021iterative}. We hope that this work will lead to more comprehensive empirical evaluation of synthetic data algorithms in subsequent work on the topic. 

\paragraph*{\textbf{[R2] Contributions and other comments}}
One contribution of the paper is a state-of-the-art mechanism with strong evidence both that it outperforms existing mechanisms and for why it performs well. The ablation shows that \aim's success is due to a combination of factors, some novel, some ``basic''. As the reviewer points out, the literature is confusing, in part because of papers that emphasize novelty, potentially at the expense of getting basic elements right and/or making all of the appropriate comparisons. We aim in this work to focus on what works well and why, and support our findings with experiments that are fair, realistic, and examine many facets of performance. We particularly appreciate the suggestions of the reviewers to add both the ablation and hyper-parameter sensitivity analyses, as these strengthen the evidence for several of our key findings.

A second contribution is easy-to-compute post hoc bounds on error, which no other synthetic data mechanism has provided, and are badly needed by practitioners.

We greatly appreciate the extensive comments of R2, which have helped us improve the paper. We addressed as many comments as we could while keeping within our vision and scope for the paper. %, but were not able to incorporate every detailed comment in our revisions.

%\ry{TODO: @Dan Sheldon, otherwise delete}

%In this work, instead of varying the degree of the marginal queries in the workload, we focused on constructing workloads that contained interesting subsets of marginals of fixed degree (in this case, 3).  We recognize that it is standard to consider workloads with non 3-way marginals, In this work, we were interested in understanding differences between workload-aware and workload-agnostic mechanisms.  To achieve that, we carefully constructed our workloads to have interesting structure that a workload-aware mechanism would be able to pick up on.  Our \target and \weighted workloads both include interesting subsets of 3-way marginals that differ from existing work that evaluates error with respect to all k-way marginals, or some simple random sample of k-way marginals.  

\paragraph*{\textbf{[R3] Justification of heuristics}}

We added more discussion to \cref{sec:aim} to better explain our choice to use a multiplicative weight of $ w_r = \sum_{s \in W} c_s | r \cap s|$ in the quality score function.  %One compelling reason to use this weighting scheme is that it makes the behavior of AIM invariant to the representation of the workload, a distinguishing feature not shared by MWEM+PGM.  For example, suppose we have two workloads, one which has two copies of the same marginal query (with weight 1) and one which has a single copy of that marginal query with weight 2.  Even though these two workloads are identical from the perspective of our error metric, the behavior of a mechanism like MWEM+PGM will be different for these two inputs, while the behavior of AIM will remain unchanged because w_r will be the same for these two representations of the same workload.  

\paragraph*{\textbf{[R3] Missing points in the plots}}

This occurred when one mechanism failed to run for the given (dataset, workload, privacy budget), and the reasons for failure differed by mechanism, ranging from timeouts, to memory usage requirements, to other runtime errors in the mechanisms.  We updated the text in \cref{sec:experiments} to point this fact out.






